Context Scaling is No Free Lunch

Large language models are increasingly trained and deployed with long contexts that span documents, code repositories, and interaction histories. This scaling implicitly treats context as a free lunch, assuming that training on longer contexts can only help the model by exposing it to richer evidence. We challenge this view by studying how the context window shapes a model's mode of learning, shifting it between parametric internalization and contextualization. We propose the Information Abundance Paradox, which hypothesizes that abundant relevant information in the training context can reduce the incentive to encode that information parametrically, thereby increasing reliance on context. In pretraining with long documents, increasing the context window improves language modeling, natural language understanding, and closed-book MCQA only up to an intermediate optimum, after which performance consistently declines. In supervised fine-tuning, more task-relevant train-time context improves performance with supporting context, but reduces robustness when context is absent or misleading at test time. Our analysis suggests that this behavior arises when longer context provides a lower complexity solution. Mechanistically, training with informative context shifts gradient pressure from feed-forward networks, often linked to parametric knowledge, toward attention modules, and causal interventions show that this shift increases reliance on context during inference. Our findings therefore suggest that context scaling is no free lunch, even when high-quality long-context data is abundant.

==> theorem_boxing_style.tex <==
% Insert in the preamble AFTER all \newtheorem definitions, BEFORE \begin{document}.
% Load dependencies here so \tcbset and \tcolorboxenvironment are defined.
\RequirePackage{xcolor}
\RequirePackage{tcolorbox}
\tcbuselibrary{skins,breakable}
% Uses the existing theorem, proposition, definition, lemma and corollary counters.
% Existing \begin{theorem}[...] ... \end{theorem} syntax is unchanged.

% Theorem / corollary: cool blue
\definecolor{resultink}{HTML}{2F4A7A}
\definecolor{resultedge}{HTML}{A9BBD6}
\definecolor{resultwash}{HTML}{F3F6FB}
% Proposition: muted ochre (warm, opposite blue)
\definecolor{propositionink}{HTML}{8A6A2F}
\definecolor{propositionedge}{HTML}{D3C29E}
\definecolor{propositionwash}{HTML}{FAF7F0}
% Definition: soft sage
\definecolor{definitionink}{HTML}{4E6B59}
\definecolor{definitionedge}{HTML}{B0C4B7}
\definecolor{definitionwash}{HTML}{F4F7F5}
% Lemma: neutral (unchanged)
\definecolor{neutraledge}{HTML}{ADB5C0}
\definecolor{neutralink}{HTML}{65717F}

\tcbset{
  formalbox/.style={
    enhanced,breakable,
    sharp corners,
    boxrule=0.45pt,
    left=9pt,right=9pt,top=8pt,bottom=7pt,
    before skip=12pt,after skip=12pt,
    before upper={\setlength{\parindent}{0pt}},
    after={\noindent},
    parbox=false
  }
}
\tcolorboxenvironment{theorem}{
  formalbox,
  colback=resultwash,
  colframe=resultedge,
  borderline west={2pt}{0pt}{resultink},
}
\tcolorboxenvironment{proposition}{
  formalbox,
  colback=propositionwash,
  colframe=propositionedge,
  borderline west={2pt}{0pt}{propositionink},
}
\tcolorboxenvironment{definition}{
  formalbox,
  colback=definitionwash,
  colframe=definitionedge,
  borderline west={2pt}{0pt}{definitionink},
}
\tcolorboxenvironment{lemma}{
  formalbox,colback=white,colframe=neutraledge,
}
\tcolorboxenvironment{corollary}{
  formalbox,colback=resultwash,colframe=resultedge,
}

% Question: dusty plum, a fourth hue next to blue, ochre and sage
\definecolor{questionink}{HTML}{6B4E71}
\definecolor{questionedge}{HTML}{CDBFD0}
\definecolor{questionwash}{HTML}{F8F5F9}

\newtcolorbox{questionbox}[1][]{
  formalbox,
  colback=questionwash,
  colframe=questionedge,
  borderline west={2pt}{0pt}{questionink},
  width=0.9\linewidth, center,
  halign=center,
  fontupper=\itshape,
  after={\par\addvspace{12pt}\noindent},
  #1
}
